The Kelvin-Helmholtz/von Neumann Stability of Discrete Representations of the Two-Fluid Model for Stratified Two-Phase Flow

Many dynamic pipe flow simulator tools are capable of predicting the onset of hydrodynamic flow instability through detailed simulation. These instabilities provide a natural mechanism for flow regime transition. The quality and reliability of flow predictions are however strongly dependent upon the numerics within these simulator tools, the scheme type and resolution in particular. A Kelvin-Helmholtz stability analysis for the differential two-fluid model is in the present work presented and extended to discrete representations of said model. This analysis provides algebraic expressions which give instantaneous, quantitative information into i) when a studied scheme will predict linear wave growth, ii) the rate of growth and the expected growing wavelength, and iii) the wave speeds. These stability expressions adhere to a wider family of finite volume methods, directly applicable to any specific formulation within this group. Both the spatial and temporal discretization are found to play decisive roles in a method's predictive capability. Fundamental aspects of how numerical errors from the temporal integration affects the predicted stability are explored. Numerical errors are observed to manifest in increased, as well as reduced, wave growth. Low-frequency growth from numerical errors is not always easily distinguished from physical wave growth. The linear analysis is demonstrated to be useful in understanding the predictions made by simulator tools, and in choosing the appropriate numerical method and simulation parameters for optimizing the simulation efficiency and reliability.

==> introduction.tex <==
\section{Introduction}

\subsection*{Literature}
Stability analysis of the two-fluid model have been preformed by numerous authors.
Barnea and Taitel used conventional stability analysis to determine stability criteria for viscous flows \cite{Barnea_VKH} and examined the non-linear flow development through simulation \cite{Barnea_simplified_with_characteristics}. The coincidence
 between the inviscid Kelvin Helmholtz (IKH) criterion and ill-posedness of the two-fluid model was established. 
Barnea also preformed a stability analysis on a discrete upwind type scheme of a simplified version of the two-fluid model for annular flow in which the gas rates were assumed to always be at a steady state \cite{Barnea_Discrete_annular_instability}. Here it was shown who an intrinsically unstable, ill-posed differential model may display stable behaviour provided sufficient numerical diffusion. (The annular interface is inherently unstable locally though may be stable in a statistical sense.) An interesting proposition that the discrete model was to be regarded as a model for the averaged flow was presented for legitimisation.
\\

Liao et. al. \cite{Liao_von_Neumann} preformed a comprehensive linear flow  stability study on a discrete two-fluid model with a staggered grid arrangement in order to determine which representation of the convection term would provide the best stability transition behaviour.
Four discretizations were teste: the central difference discretization, the `first order upwind' or `donor-cell' discritizaion, second order upwind and the QUICK discretizations. 
It was found that the central difference discretization was superior in this respect.  The study did not address High-wavenumber numerical issues associated with central difference convection, such as the Gibbs oscillation phenomena associated with discontinuities.
\\

The doctoral thesis of Renault~\cite{LASSI} contained a stability analysis on a particular upwind type, staggered grid discretization of the two-fluid model. The spatial numerical diffusion and dispersion effects were included into a extended dispersion equation to yield a stability criterion analogous to the VKH criterion for this upwind scheme. The resulting criterion was valid for low wavenumbers only.


\subsection*{Motivation}
A full picture of the linear stability properties of the two-fluid model is still wanting.  
%Most discrete stability analysis are scheme specific and render little understanding of how the numerous discretization decision will influence the flow stability properties when representing the two-fluid model numerically. 
In this work some effort is put into mapping out the effect of various discretization choices, in particular the choices between 
\begin{itemize}
\setlength{\itemsep}{-3pt}
	\item staggered and non-staggered grid arrangements,
	\item conservative and non-conservative forms of the two-fluid model, 
	\item tern discretization (centred vs. upwind),
	\item influence of artificial diffusion terms,
	\item simplifications to the two-fluid model itself, 
	%\item two-equation and four-equation schemes, and
	\item various scheme reductions.
\end{itemize}

Concrete quantitative stability criteria for numerous schemes provide the opportunity to more precisely choose a discretization that is  suited both in terms of flow and numerical stability. Precise knowledge of when a discrete representation will predict hydrodynamically unstable flow may also be useful in the computational treatment of flow regime transitions, and it provides quantitative resolution requirements for so-called hydrodynamic wave or slug capturing.


\subsection*{Limitations}
It is proper to clearly remark on the main limitations of this analysis right form the beginning.
\\
Foremost, the linear stability analysis is technically only valid in the limit of infinitesimal disturbances, and it gives on indication of the flow development beyond the initial growth. A practical consequence of this linearisation is that some of the discretization details, those that are manifested in a higher order of the disturbance, falls out.   

Secondly, one of the principle assumptions throughout this article is that of incompressibility regarding both phases. This effectively excludes all issues concerning numerical treatment of the pressure terms, such as stencils for the pressure and the well-know problem alternate high-wavenumber solutions (checkerboard solutions.)






%
%
%
%\section{The Two-Fluid Model}
%
%
%
%The two-fluid model for stratified flow is commonly written
%\begin{subequations}
%\begin{align}
%\label{eq:system:mass}
%&\partial_t\brac{\rho \adyn}\kap + \partial_x\brac{\rho \adyn u}\kap = 0,
%\\
%\label{eq:system:momentum}
%&\partial_t\brac{\rho \adyn u}\kap + \partial_x\brac{\rho \adyn u^2}\kap + \rho\kap \adyn\kap g \cos\theta \partial_xh\l 
%+\adyn\kap \partial_xp\^i= \mcs\kap.
%\\
%&\adyn\l+\adyn\g = A
%\end{align}
%\label{eq:system}
%\end{subequations}
%%
%There exists a vast number of ways in which to represent \eqref{eq:system} discretely. Here, the representations chosen are those that become unambiguous in a linear stability analysis when discretising with the most basic techniques. 
%
%This linear stability analysis rests on the assumption of incompressible phases which allows for the pressure gradient to be eliminated directly. The pressure gradient is eliminated by dividing each momentum equation with their respective phase fraction and subtracting the two. The phase fraction identity $\al+a\g=A$ then reduces \eqref{eq:system} to a two-equation system. If this reduction is made after or before discretisation makes little difference in terms of the linear stability criteria, but it is easier to avoid ambiguities if the reduced two-equation differential system is approached directly. Numerical treatment of the pressure term therefore falls outside the scope of what is examined with linear analysis in the incompressible case. 
%
%
%
%After incompressible reduction to its two-equation form, system \eqref{eq:system} reads
%\begin{equation}
%\partial_t  \adyn\l + \partial_x\brac{\adyn u}\l = 0,
%\label{eq:system:mass}
%\end{equation}
%%
%%\nolinebreak
%\begin{subequations}
%\begin{align}
%%\frac{\partial_t \brac{\rho\adyn u}\l}{\adyn\l} 
%%-\frac{\partial_t \brac{\rho\adyn u}\g}{\adyn\g} 
%%+\frac{\partial_x \brac{\rho\l\adyn\l u\l^2 + \frac12 \rho\l \frac{\adyn\l^2}{\adyn\l'} g \cos\theta}}{\adyn\l} 
%%-\frac{\partial_x \brac{\rho\g\adyn\g u\g^2 + \frac12 \rho\g \frac{\adyn\g^2}{\adyn\g'} g \cos\theta}}{\adyn\l}
%%\diffk{\frac{\partial_t \rho\adyn u}{\adyn}}
%%+\diffk{\frac{\partial_x \brac{\rho\adyn u^2 + \frac12 \rho \frac{\adyn\l^2}{\adyn\l'} g \cos\theta}}{\adyn} }
%%&= \mcs ,
%\diffk{\frac{\partial_t \rho\adyn u}{\adyn}}
%+\diffk{\frac{\partial_x \rho\adyn u^2}{\adyn} + \rho  g \cos\theta\,   \partial_x h }
%&= \mcs ,
%%\\
%%\diffk{\frac{\rho\,\partial_t \adyn u}{\adyn}}
%%+\diffk{\frac{\rho\,\partial_x \adyn u^2 +  \rho g \cos\theta \frac 12 \frac{\partial_x\adyn\l^2}{\adyn\l'} }{\adyn} }
%%&= \mcs ,
%\label{eq:system:subtracted_momentum:NR}
%\\
%%
%%\partial_t \sqbrac{\brac{\rho u}\l-\brac{\rho u}\g}
%%+\partial_x \sqbrac{\rho\l \frac {u\l^2}2-\rho\g \frac {u\g^2}2 + \brac{\rho\l-\rho\g} \frac{\adyn\l}{\adyn\l'} g \cos\theta}
%%\partial_t \diffk{\rho u}
%%+\partial_x \brac{\diffk{\rho \frac {u^2}2} + \diffk{\rho} \frac{\adyn\l}{\adyn\l'} g \cos\theta}
%%&= \mcs,
%%\\
%\partial_t \diffk{\rho u}
%+\partial_x \brac{\diffk{\rho \frac {u^2}2} + h  \diffk{\rho}  g \cos\theta}
%&= \mcs,
%\label{eq:system:subtracted_momentum:R}
%\end{align}
%\label{eq:system:subtracted_momentum}
%\end{subequations}
%with $\adyn\k'=\ddiff{\adyn\k}{h\l}$ and $\mcS\k = -\tau\k\Sigma\k - \tau\k\^i\Sigma\k\^i
%- \rho\k \adyn\k g \sin\theta$. 
%Equation~\eqref{eq:system:subtracted_momentum:NR} originates straight form \eqref{eq:system:momentum} while Equation~\eqref{eq:system:subtracted_momentum:R} is the conservative form obtained by reduction with \eqref{eq:system:mass}.
%The form \eqref{eq:system:subtracted_momentum:NR} will typically represent the full form  \eqref{eq:system:momentum} where the pressure is treated with precision (typically through in iterative pressure correction method, \egg\ Patankar's SIMPLE method.) From \eqref{eq:system:subtracted_momentum:R} best represents an incompressible system where the model equations have been reduced to this form.
%
%In addition, the summation of $\kappa=\ell,\mr g$ in \eqref{eq:system:mass} yields the constant mixture velocity condition 
%\begin{equation}
%%	\ag u\g  + \al u\l = \Um\of t.
%	u\g\^S  + u\l\^S = \Um\of t,
%\label{eq:Um}
%\end{equation}
%closing the system.
%Superficial velocities are defined $u\k\^S = \frac{a\k}{a}u\k$.
%
%
%
%
%The friction model $s\k$ is based on the rather simple Taitel and Dukler model \cite{Taitel_Dukler_friction_factor} quickly summarised below:
%\begin{gather}
%	s\k = -\sigma\k \tau\k + \sigma\_i \tau_{\mr i,k} - \ak \rho\k g \sin\!\theta,
%	\label{eq:s}
%	\\
%	\nonumber
%	\begin{aligned}
%		&\tau\k = \nicefrac12 \fric\k \rho\k u\k |u\k|,
%		&
%		&\tau\_{i,\ell} = -\tau\_{i,g} = \tau\_i ,
%		\\
%		&\tau\_i = \nicefrac12 \fric\_i \rho\g(u\g-u\l)|u\g-u\l|,
%		&
%		&\fric\k = c\k (u \, d/\nu)\k^{-n\k},
%		\\
%	%	Re_{\mr D,k} &= (u D/\nu)\k
%	%	&
%		&d\l = 4\, a\l/\sigma\l,
%		&
%		&d\g = 4\, a\g/(\sigma\l+\sigma\_i).
%	\end{aligned}
%\end{gather}
%%\begin{gather*}
%%	s\k = -\Sigma\k \tau\k/A + \Sigma\_i \tau_{\mr i,k}/A - \ak \rho\k g \cos\phi
%%	\\
%%	\begin{tabular}{ccc}
%%		$\tau\k = \nicefrac12 \fric\k \rho\k u\k |u\k|$
%%		&
%%		$\tau\_{i,\ell} = -\tau\_{i,g} = \tau\_i $
%%		\\
%%		$\tau\_i = \nicefrac12 \fric\_i \rho\g(u\g-u\l)|u\g-u\l|$
%%		&
%%		$\fric\k = c\k (u D/\nu)\k^{-n\k}$
%%		\\
%%	%	Re_{\mr D,k} &= (u D/\nu)\k
%%	%	&
%%		$D\l = 4 A\l/\Sigma\l$
%%		&
%%		$D\g = 4 A\g/(\Sigma\l+\Sigma\_i)$
%%	\end{tabular}
%%\end{gather*}
%The coefficients $c\l$ and $c\g$ equal $0.046$ for turbulent flow and $16$ for laminar, while $n\l$ and $n\g$ equal $0.2$ for turbulent flow and $1.0$ for laminar flow. The interfacial friction factor is $f\_i=m\_x\max\{f\g, 0.014\}$. $m\_x$ is here a type of correction parameter employed by numerous authors to achieve $f\_i > f\g$ as observed experimentally.
%%As suggested varies for $m_x$ varies it is in the present work fixed to a value $5.0$, the interface friction model being rather rudimentary anyway.
%A study on how $m\_x$ affect the wave regime was carried out in \cite{George_PhD} and will not be repeated here.
%Here, $m\_x=5.0$ is chosen together with air-water properties at atmospheric conditions. This provides an acceptable range within which the two-fluid model predicts roll wave formations. The quasi-steady roll wave formations will later be used to study the non-linear stability properties of the discrete representations.
%% Instead $m\_x$ is rather arbitrarily given the value $m\_x=5.0$.
%\\
%
%The friction model here presented and used is not a good physical representation of all those physical effects arising in wavy stratified flow. Nor is it intended to be. It does no the other hand scale the friction to an appropriate magnitude. 
%%
%%The friction model implemented herein does not take any account of wave breaking phenomena and the like.
% More elaborate friction models, carrying physical effects from the turbulent flow profile through the rough cross-sections are provided in Biberg's work \cite{Biberg_friction_duct_2007}.%,Biberg_frictio
%A study on reliable roll wave predictions is given by Holm{\aa}s in \cite{Holmaas_roll_wave_model}.
%%The author recommends \cite{Biberg_friction}. Other friction factor models, such as H{\aa}land's explicit expression, can also be used.
%%Good examples are  H{\aa}land's explicit expression for friction in rough pipes or Biberg's \cite{Biberg_friction_duct_2007}%,Biberg_friction_pipe_2000} 
%% turbulent friction models based on pre-integration of stratified flow profiles over the cross-section.
%
%



==> nomenclature.tex <==
 
% Latin
\nomenclature[Aa]{$a\k,A\k$ }{Cross-sectional area occupied by phase $\kappa$ \nomunit{m^\textrm{2}} }%
\nomenclature[Au]{$u\k,U\k$ }{Fluid velocity \nomunit{m\,s^\textrm{-1}} }%
\nomenclature[Ah]{$h\k$ }{Level height \nomunit{m} }%
\nomenclature[Ag]{$G$ }{Amplification factor \nomunit{\cdot}  }%
\nomenclature[Au]{$k$ }{Wavenumber \nomunit{m^\textrm{-1}} }%
\nomenclature[Ac]{$C$ }{Wave velocity \nomunit{m\,s^\textrm{-1}} }%
\nomenclature[As]{$\mcS$ }{Source term (viscous friction, gravity) \nomunit{kg\,m^\textrm{-1}} }%
\nomenclature[Ar]{$\mc R_{C^m}$ }{Wave dispersion equation coefficients \nomunit{kg\,m^\textrm{-3}} }%
\nomenclature[Aq]{$q$}{Time integration switch ($+1$ for implicit, $-1$ for explicit)\nomunit{\cdot}}

%Greek
\nomenclature[B01]{$\alpha$}{Phase fraction \nomunit{\cdot} }%
\nomenclature[B17]{$\rho$}{Density \nomunit{kg\,m^\textrm{-3}} }%
\nomenclature[B21]{$\phi$}{Phase angle \nomunit{\cdot} }%
\nomenclature[B23]{$\psi$}{Generic variable \nomunit{-} }%
\nomenclature[B24]{$\omega$}{Angular frequency/pulsation \nomunit{s^\textrm{-1}} }%
\nomenclature[B19]{$\LF$}{Artificial numerical diffusion \nomunit{\cdot} }%
\nomenclature[B19]{$\UW$}{Upwind weighting factor \nomunit{\cdot} }%
\nomenclature[B08]{$\theta$}{Elevation angle \nomunit{\cdot} }%

% Subscripts
\nomenclature[Ck0]{$\kappa$}{Phase index, $\sigma\in\{\mathrm{g,\ell}\}$}%
\nomenclature[Cj0]{$j$}{Spatial node index}%
\nomenclature[C0]{$0$}{Evaluated at steady state.}%
\nomenclature[Cv0]{iv}{Inviscid}%
\nomenclature[Cv1]{v}{Viscous}%
\nomenclature[Ci]{i, r}{Imaginary, real.}%

% Superscripts
\nomenclature[Ds]{ S }{Superficial quantity}
\nomenclature[Dn1]{ $n$ }{Time iteration index}
\nomenclature[Dn2]{ $n+\h$ }{Symbolic time iteration index, dependent upon the time integration strategy}
\nomenclature[Da]{$*$}{Critical value -- at stability limit.}%


% Encasements
\nomenclature[E1]{$\ol{(\cdot)}$ }{Arithmetic average of left and right state}% cf.\ Equation~\eqref{eq:upwind}}%

%abbreviations
\nomenclature[F1]{ IKH }{`Inviscid Kelvin Helmholtz'}%
\nomenclature[F1]{ VKH }{`Viscous Kelvin Helmholtz'}%
\nomenclature[F2]{ CD }{`Central Difference'}%
\nomenclature[F2]{ UW }{`Upwind'}%
\nomenclature[F2]{ LF }{`Lax-Friedrich' (artificial numerical diffusion)}%
\nomenclature[F3]{ S, NS }{`Staggered, Non-Staggered' (grid)}%
\nomenclature[F3]{ C, NC }{`Conservative, Non-Conservative' (formulation)}%
